Learning to Play Imperfect-Information Games by Imitating an Oracle Planner

We consider learning to play multiplayer imperfect-information games with simultaneous moves and large state-action spaces. Previous attempts to tackle such challenging games have largely focused on model-free learning methods, often requiring hundreds of years of experience to produce competitive agents. Our approach is based on model-based planning. We tackle the problem of partial observability by first building an (oracle) planner that has access to the full state of the environment and then distilling the knowledge of the oracle to a (follower) agent which is trained to play the imperfect-information game by imitating the oracle's choices. We experimentally show that planning with naive Monte Carlo tree search does not perform very well in large combinatorial action spaces. We therefore propose planning with a fixed-depth tree search and decoupled Thompson sampling for action selection. We show that the planner is able to discover efficient playing strategies in the games of Clash Royale and Pommerman and the follower policy successfully learns to implement them by training on a few hundred battles.

==> fdts.tex <==


\subsection{Decoupled Thompson sampling}

%An instance of UCB for player $i \in N$ in state $s$ is used to independently choose actions from $A_i(s)$.
%UCB algorithms are the most popular choice for action selection in multi-armed bandit problems \cite{browne2012survey, silver2017mastering}. UCB algorithms estimate the upper confidence bound that any given action is optimal. 
%While there exists different variations of UCB algorithms, we consider the commonly used UCB1 variant introduced in \cite{auer2002finite}. 
The most common action selection algorithm used in simultaneous-move MCTS is Decoupled UCB (upper confidence bound) \cite{auer2002using}. In Decoupled UCB, each node in the tree consists of independent instances of UCB % \cite{auer2002using}
for each player. 
Each player $i$ independently estimates the upper confidence bound %$\UCB_i(s, a_i)$
for each action $a_i \in A_i(s)$ as
\[ \UCB_i(s, a_i) = Q_i(s, a_i) + c \sqrt{\frac{\log N}{n_{a_i}}} \,, \]
%$ \UCB_i(s, a_i) = Q_i(s, a_i) + c \sqrt{\frac{\log N}{n_{a_i}}} \,, $
where the hyperparameter $c$ controls the exploration-exploitation trade-off, $n_{a_i}$ is the visit count of action $a_i$ and $N = \sum_{a_i \in A_i(s)} n_{a_i}$.
However, we found it difficult to tune the exploration parameter $c$ of UCB for games
with large and dynamic action spaces (such as Clash Royale), in which the number of actions available in each state varies a lot.

%In each iteration, the action with the highest UCB value is chosen deterministically. At the end of planning, normalized visit counts define a probability distribution over actions. The final action can be chosen stochastically by sampling from this distribution of by deterministically choosing the action with the highest visit count.

%\subsection{Thompson Sampling (TS)}

We therefore propose to use decoupled Thompson sampling as a solution which naturally handles the exploration-exploitation trade-off %in large dynamic action spaces
without any hyperparameter tuning.
%Introduced by \citet{thompson1933likelihood}, 
Thompson sampling \cite{thompson1933likelihood} maintains probability distributions of cumulative rewards for each action and chooses actions proportional to the probability that they are optimal. 
%Thompson sampling was largely ignored until strong empirical results were recently presented in \cite{scott2010modern, chapelle2011empirical}. Since then, it has been well studied and applied to diverse problems \cite{ortega2010minimum, russo2014learning, russo2018tutorial}.
Since the rewards in Clash Royale and Pommerman are binary,
%based on winning or losing
the probability that each action $a_i$ is optimal is modeled using Bernoulli distributions with mean $\theta^*_{a_i}$. 
The means $\theta^*_{a_i}$ %of these Bernoulli distributions
can be modeled using conjugate Beta distributions,
%, as Beta distribution is the conjugate prior for Bernoulli distribution. This can be
which is implemented by maintaining win and loss counts ($S_{a_i}$ and $F_{a_i}$ respectively) for each action.
%(we assume a draw to be both a win and a loss). 
Note that this posterior update assumes independent samples from a Bernoulli distribution, even though this is not true in a multi-agent setting.
During each iteration of planning, the action is chosen as
%$ a_i = \argmax_{a_i \in A_i(s)} \theta_{a_i} \,, $
%such that
%$ \theta_{a_i} \sim \Beta(S_{a_i} + \alpha, F_{a_i} + \beta) \,, $
\[ a_i = \argmax_{a_i \in A_i(s)} \theta_{a_i} \,,
\qquad
\theta_{a_i} \sim \Beta(S_{a_i} + \alpha, F_{a_i} + \beta) \,.
\]
%where $\alpha$ and $\beta$ are the priors of the Beta distribution.
In all the experiments in the paper, we set $\alpha=\beta=1$ and do not tune these hyperparameters. At the end of planning, the final action can be chosen stochastically in a similar manner by sampling or deterministically based on the estimated means of the Beta distributions.
%\[ a_i = \argmax_{a_i \in A_i(s)} \frac{S_{a_i} + \alpha}{S_{a_i} + F_{a_i} + \alpha + \beta} \]


\begin{enumerate}

\item \textbf{Selection.} In state $s$, both players independently choose actions $a_i \in A_i(s)$ based on a MAB algorithm which leads the battle to a new state $s'$. Action selection in the new state $s'$ is also performed similarly using the same MAB algorithm. Nodes are added to the search tree corresponding to all encountered states with the edges corresponding to joint action taken to reach the state. Each node consists of an instance of an MAB algorithm used to perform action selection in that state/node. 
\item \textbf{Expansion.} From root state $s$, the selection step continues until it reaches a newly encountered state $\tilde{s}$ (that is, a state with no corresponding node in the search tree). A new leaf node is added to the search tree to represent the new state $\tilde{s}$.

\item \textbf{Evaluation.} This step involves estimating the value $V(\tilde{s})$ of state $\tilde{s}$ \eqref{eq:v}. This can be performed by: 1) random rollout(s) from state $\tilde{s}$ until the battle reaches a terminal state $z$ (the outcome $R(z)$ is a Monte Carlo estimate of the value), 2) a handcrafted value function, or 3) a learned value function (one can train a function approximator to predict the expected outcome of the game from any state).
{\bf discuss how this is done in CR and P.}

\item \textbf{Backup.} Instances of MAB algorithms corresponding to all states encountered in an iteration are updated based on the value estimate $V(\tilde{s})$ to make better choices in future iterations.

\end{enumerate}

\subsection{Fixed-Depth Tree Search (FDTS)}

MCS described previously has several limitations: 1) it only plans actions for the current state and hence cannot discover effective action combinations, 2) it discards all information about future states and actions traversed during rollouts and plans from scratch in each step, and 3) the rollout policy is random and hence the estimated 
%$\UCB$ or 
$Q$ values are under the assumption that both players will act randomly in the future. 
%The problems can be effectively mitigated by using Monte Carlo Tree Search (MCTS) \cite{coulom2006efficient}.
%\subsection{Standard MCTS}
%\label{s:mcts}
The problems can be effectively mitigated by using tree search, that is, building a tree of all states visited during rollouts and considering action selection in these states as a multi-armed bandit problem. We propose to perform fixed-depth rollouts in each iteration and refer to this algorithm as Fixed-Depth Tree Search (FDTS).
Each iteration of FDTS begins from the root node corresponding to current state $s$ and proceeds with the following three steps:
%FDTS builds upon MCS by considering action selection in all states encountered during rollouts as a multi-armed bandit problem.
%MCTS is a best-first tree search algorithm and begins from a root node corresponding to current state $s$. We start with the most common variant of MCTS in which each MCTS iteration from current state $s$ consists of four steps:

\begin{enumerate}
\item \textbf{Selection.} In state $s$, both players independently choose actions $a_i \in A_i(s)$ based on a MAB algorithm which leads the battle to a new state $s'$. Action selection in the new state $s'$ is also performed similarly using the same MAB algorithm. Nodes are added to the search tree corresponding to all encountered states with the edges corresponding to joint action taken to reach the state. Each node consists of an instance of an MAB algorithm used to perform action selection in that state/node. This is repeated for a fixed number of times to reach state $\tilde{s}$, that is, till we reach a fixed depth in the search tree.

%\item \textbf{Expansion.} From root state $s$, the selection step continues until it reaches a newly encountered state $\tilde{s}$ (that is, a state with no corresponding node in the search tree). A new leaf node is added to the search tree to represent the new state $\tilde{s}$.

\item \textbf{Evaluation.} This step involves estimating the value $V(\tilde{s})$ of state $\tilde{s}$ (Equation~\ref{eq:v}). This can be performed by: 1) random rollout(s) from state $\tilde{s}$ until the battle reaches a terminal state $z$ (the outcome $R(z)$ is a Monte Carlo estimate of the value), 2) a handcrafted value function, or 3) a learned value function (one can train a function approximator to predict the expected outcome of the game from any state).

\item \textbf{Backup.} Instances of MAB algorithms corresponding to all states encountered in an iteration are updated based on the value estimate $V(\tilde{s})$ to make better choices in future iterations.

\end{enumerate}

After several planning iterations, both players independently choose their best actions and the search tree built by FDTS is re-used for planning in subsequent states by moving the root node to the child node corresponding to the chosen joint action. FDTS allows for discovery of effective sequence of actions, reuse of statistics computed from previous states and iterative improvement of the rollout policy.


==> figure.tex <==
\begin{tikzpicture}[node distance=8mm, thick, scale=1.0, every node/.style={scale=1.0}]

\path[use as bounding box] (-15mm,-35mm) rectangle (45mm,30mm);

\small
\draw
      
node at (0,0)[layer, node distance=23mm, minimum width=25mm, minimum height=10mm] (oracle) {Oracle}
node [layer, right of=oracle, node distance=22mm, minimum height=10mm] (f1) {\shortstack{Player 1\\(follower)}}
node [layer, right of=f1, node distance=15mm, minimum height=10mm] (f2) {\shortstack{Player 2\\(follower)}}

node at ($(oracle)!0.28!(f1) + (0, 25mm)$)[inner sep=0] (s1) {\includegraphics[width=7mm]{giant_archer.png}}  % 14mm
node at ($(s1) + (15mm, 0)$)[inner sep=0] (s2)
{\includegraphics[width=7mm,angle=180,origin=c]{giant_archer.png}}  % 14mm

%node at ($(f1)!0.5!(f2)$)[layer, above=8mm] (o1) {Observations}

node [above of=f1, node distance=8mm] {$o_1$}
node [above of=f2, node distance=8mm] {$o_2$}

node at ($(oracle.center) + (-7mm, 8mm)$) {$o_1$}
node at ($(oracle.center) + (7mm, 8mm)$) {$o_2$}

node at ($(f1.south)+(-8mm, -6mm)$) (pf1){
\begin{axis}[
    ytick=\empty, xtick=\empty,
    area style, width=25mm, height=20mm,
    axis line style={draw=none}, tick style={draw=none},
]
\addplot+[ybar interval,mark=no] plot coordinates {(0, 3) (1, 5) (2, 4) (3, 4) (4, 2) (5, 3) (6, 1) };
\end{axis}
}
node at ($(f1.south west) + (1.9mm, -4mm)$) (pi1) {$Q_1$}

node at ($(f2.south)+(-8mm, -6mm)$) (pf2){
\begin{axis}[
    ytick=\empty, xtick=\empty,
    area style, width=25mm, height=20mm,
    axis line style={draw=none}, tick style={draw=none},
]
\addplot+[ybar interval,mark=no] plot coordinates {(0, 1) (1, 5) (2, 2) (3, 4) (4, 5) (5, 1) (6, 1) };
\end{axis}
}
node at ($(f2.south west) + (1.9mm, -4mm)$) (pi2) {$Q_2$}

%%% MCTS
node at ($(oracle.south) + (0, -1mm)$)[inner sep=0] (root){}
node at ($(root)+(-4mm, -8mm)$)[inner sep=0] (c11){}
node at ($(root)+(4mm, -8mm)$)[inner sep=0] (c12){}

node at ($(c11)+(-2mm, -4mm)$)[inner sep=0] (c21){}
node at ($(c11)+(2mm, -4mm)$)[inner sep=0] (c22){}

node at ($(c12)+(-2mm, -4mm)$)[inner sep=0] (c23){}
node at ($(c12)+(2mm, -4mm)$)[inner sep=0] (c24){}

node at ($(c21)+(-2mm, -4mm)$)[inner sep=0] (c31){}
node at ($(c21)+(2mm, -4mm)$)[inner sep=0] (c32){}

node at ($(c22)+(-2mm, -4mm)$)[inner sep=0] (c33){}
node at ($(c22)+(2mm, -4mm)$)[inner sep=0] (c34){}

node at ($(c23)+(-2mm, -4mm)$)[inner sep=0] (c35){}
node at ($(c23)+(2mm, -4mm)$)[inner sep=0] (c36){}

node at ($(c24)+(-2mm, -4mm)$)[inner sep=0] (c37){}
node at ($(c24)+(2mm, -4mm)$)[inner sep=0] (c38){}


node at ($(c32)+(-9mm, -5mm)$) (p1){
\begin{axis}[
    ytick=\empty, xtick=\empty,
    area style, width=25mm, height=20mm,
    axis line style={draw=none}, tick style={draw=none},
]
\addplot+[ybar interval,mark=no] plot coordinates {(0, 2) (1, 6) (2, 3) (3, 5) (4, 1) (5, 4) (6, 1) };
\end{axis}
}

node at ($(c36)+(-8mm, -5mm)$) (p2){
\begin{axis}[
    ytick=\empty, xtick=\empty,
    area style, width=25mm, height=20mm,
    axis line style={draw=none}, tick style={draw=none},
]
\addplot+[ybar interval,mark=no] plot coordinates {(0, 2) (1, 4) (2, 3) (3, 5) (4, 4) (5, 2) (6, 2) };
\end{axis}
}

;

%\draw [->,>=stealth](s1.south) -- node {} (s1.south|-oracle.north);
%\draw [->,>=stealth](s2.south) -- node {} (s2.south|-oracle.north);
\draw [->,>=stealth](s1.south) -- node {} ([xshift=-7mm]oracle.north);
\draw [->,>=stealth](s2.south) -- node {} ([xshift=+7mm]oracle.north);

%\draw [->,>=stealth]([yshift=-3mm]s1.south) -| node {} (f1.north);
%\draw [->,>=stealth]([yshift=-6mm]s2.south) -| node {} (f2.north);
\draw [->,>=stealth](s1.south) -- node {} (f1.north);
\draw [->,>=stealth](s2.south) -- node {} (f2.north);

% MCTS
\draw [->,>=stealth,thin](root) -- node {} (c11);
\draw [->,>=stealth,thin](root) -- node {} (c12);

\draw [->,>=stealth,thin](c11) -- node {} (c21);
\draw [->,>=stealth,thin](c11) -- node {} (c22);

\draw [->,>=stealth,thin](c12) -- node {} (c23);
\draw [->,>=stealth,thin](c12) -- node {} (c24);

\draw [->,>=stealth,thin](c21) -- node {} (c31);
\draw [->,>=stealth,thin](c21) -- node {} (c32);

\draw [->,>=stealth,thin](c22) -- node {} (c33);
\draw [->,>=stealth,thin](c22) -- node {} (c34);

\draw [->,>=stealth,thin](c23) -- node {} (c35);
\draw [->,>=stealth,thin](c23) -- node {} (c36);

\draw [->,>=stealth,thin](c24) -- node {} (c37);
\draw [->,>=stealth,thin](c24) -- node {} (c38);

\draw [->,>=stealth](s2.east) -- node {} ++(35mm, 0);

\draw [->,>=stealth,rounded corners=10pt]([xshift=2mm,yshift=-8mm]f2.south) -- ++(0, -3mm) -| ([xshift=5mm, yshift=-5mm]f2.east|-s2.east) node[above] {$a_2$};
\draw [->,>=stealth,rounded corners=10pt]([xshift=2mm,yshift=-8mm]f1.south) -- ++(0, -5mm) -| ([xshift=9mm, yshift=-5mm]f2.east|-s2.east) node[above] {$a_1$};

\draw [->,>=stealth,dashed]([xshift=8mm,yshift=0mm]p2.south) -- ++(0, -3mm) -| ([xshift=-1mm, yshift=-7mm]f2.south);
\draw [->,>=stealth,dashed]([xshift=8mm,yshift=0mm]p1.south) -- ++(0, -5mm) -| ([xshift=-1mm, yshift=-7mm]f1.south);

\end{tikzpicture}
